Temporal network analysis: Introduction, methods and detailed tutorial with R

Learning involves relations, interactions and connections between learners, teachers and the world at large. Such interactions are essentially temporal and unfold in time. Yet, researchers have rarely combined the two aspects (the temporal and relational aspects) in an analytics framework. Temporal networks allow modeling of the temporal learning processes i.e., the emergence and flow of activities, communities, and social processes through fine-grained dynamic analysis. This can provide insights into phenomena like knowledge co-construction, information flow, and relationship building. This chapter introduces the basic concepts of temporal networks, their types and techniques. A detailed guide of temporal network analysis is introduced in this chapter, that starts with building the network, visualization, mathematical analysis on the node and graph level. The analysis is performed with a real-world dataset. The discussion chapter offers some extra resources for interested users who want to expand their knowledge of the technique.

==> references.tex <==

@misc{Bender-deMoll_2016, title={Temporal network tools in statnet: networkDynamic, ndtv and tsna}, url={https://web.archive.org/web/20180423112846/http://statnet.csde.washington.edu/workshops/SUNBELT/current/ndtv/ndtv_workshop.html}, journal={statnet}, author={Bender-deMoll, Skye}, year={2016} }

@article{Bender-deMoll_2018, title={ndtv: Network Dynamic Temporal Visualizations}, url={https://cran.r-project.org/package=ndtv}, author={Bender-deMoll, Skye}, year={2018}, annote={R package version 0.12.3} }

@article{Bender-deMoll_Morris_2016, title={tsna: Tools for temporal social network analysis}, journal={R package version 0.2. 0, URL https://CRAN. R-project. org/package= tsna}, author={Bender-deMoll, Skye and Morris, Martina}, year={2016} }

@article{Brey_2018, title={Temporal network analysis with R}, ISSN={2397-2068}, url={http://dx.doi.org/10.46430/phen0080}, DOI={10.46430/phen0080}, abstractNote={Learn how to use R to analyze networks that change over time.}, number={7}, journal={The programming historian}, publisher={University of Sussex}, author={Brey, Alex}, year={2018}, month={Nov}, language={en} }

@book{Butts_Leslie-Cook_Krivitsky_Bender-Demoll_2014, title={Dynamic extensions for network objects}, author={Butts, C. T. and Leslie-Cook, A. and Krivitsky, P. N. and Bender-Demoll, S.}, year={2014} }

@article{Chen_Poquet_2020, title={Socio-temporal dynamics in peer interaction events}, abstractNote={Asynchronous online discussions are broadly used to support peer interaction in online and hybrid courses. In this paper, we argue that the analysis of online peer interactions would benefit from the focus on relational events that are temporal and occur due to a range of factors. To demonstrate the possibility, we applied Relational Event Modeling (REM) to a dataset from online discussions in seven online classes. Informed by a conceptual model of social interaction in online discussions, this modeling included (a) a learner attribute capturing aspects of temporal participation, (b) social dynamics factors such as preferential attachment and reciprocity, and (c) turnby-turn sequential patterns. Results showed that learner activity and familiarity from recent interactions affected their propensity to form ties. Turn-by-turn sequential patterns, that capture individual posting in bursts, explain how two-star network patterns form. Since two-star network patterns could further facilitate small group formation in the network, we expected the models to also capture communication in triads (i.e. triadic closure). Yet, models, devoid of the content of exchanges, did not capture the social dynamics well, and failed to predict patterns for communication across triads. By bringing in discourse features, future work can investigate the role of knowledge building behaviours in triadic closure of digital networks. This study contributes fresh insights into social interaction in online discussions, calls for attention to micro-level temporal patterns, and motivates future work to scaffold learner participation in similar contexts.}, journal={ACM International Conference Proceeding Series}, author={Chen, Bodong and Poquet, Oleksandra}, year={2020}, pages={203–208}, keywords={Digital peer networks; Relational event modelling; Temporality} }

@inproceedings{Chen_Wise_Knight_Cheng_2016, title={Putting temporal analytics into practice: the 5th international workshop on temporality in learning data}, ISBN={9781450341905}, booktitle={Proceedings of the sixth international conference on learning analytics & knowledge}, publisher={ACM}, author={Chen, Bodong and Wise, Alyssa F. and Knight, Simon and Cheng, Britte Haugan}, year={2016}, pages={488–489} }

@article{Elmoazen_Saqr_Tedre_Hirsto_2022, title={A systematic literature review of empirical research on epistemic network analysis in education}, volume={10}, ISSN={2169-3536}, journal={IEEE access: practical innovations, open solutions}, publisher={Institute of Electrical and Electronics Engineers (IEEE)}, author={Elmoazen, Ramy and Saqr, Mohammed and Tedre, Matti and Hirsto, Laura}, year={2022}, pages={17330–17348} }

@misc{Heikkinen_Lopez-Pernas_Malmberg_Tedre_Saqr, title={How do business students self-regulate their project management learning? A sequence mining study}, url={https://ceur-ws.org/Vol-3383/FLAIEC22_paper_2583.pdf}, author={Heikkinen, Sami and Lopez-Pernas, Sonsoles and Malmberg, Jonna and Tedre, Matti and Saqr, Mohammed} }

@article{Hernández-García_González-González_Jiménez-Zarco_Chaparro-Peláez_2015, address={["Departamento de Ingeniería de Organización, Administración de Empresas y Estadística, Universidad Politécnica de Madrid, Madrid, Spain", “Estudis d’Economia i Empresa, Universitat Oberta de Catalunya, Barcelona, Spain”, "Economics and Business Studies,}, title={Applying social learning analytics to message boards in online distance learning: A case study}, volume={47}, ISSN={0747-5632}, abstractNote={Social learning analytics introduces tools and methods that help improving the learning process by providing useful information about the actors and their activity in the learning system. This study examines the relation between SNA parameters and student outcomes, between network parameters and global course performance, and it shows how visualizations of social learning analytics can help observing the visible and invisible interactions occurring in online distance education. The findings from our empirical study show that future research should further investigate whether there are conditions under which social network parameters are reliable predictors of academic performance, but also advises against relying exclusively in social network parameters for predictive purposes. The findings also show that data visualization is a useful tool for social learning analytics, and how it may provide additional information about actors and their behaviors for decision making in online distance learning.}, number={PG-68-80}, journal={Computers in human behavior}, publisher={Elsevier Ltd}, author={Hernández-García, Ángel and González-González, Inés and Jiménez-Zarco, Ana Isabel and Chaparro-Peláez, Julián}, year={2015}, month={Jun}, pages={68–80}, keywords={Data visualization; Learning analytics; Online distance learning; Social learning analytics; Social network analysis}, language={English}, annote={From Duplicate 2 (Applying social learning analytics to message boards in online distance learning: A case study - Hernández-García, Ángel; González-González, Inés; Jiménez-Zarco, Ana Isabel; Chaparro-Peláez, Julián) From Duplicate 1 (Applying social learning analytics to message boards in online distance learning: A case study - Hernández-García, Ángel; González-González, Inés; Jiménez-Zarco, Ana Isabel; Chaparro-Peláez, Julián) From Duplicate 1 (Applying social learning analytics to message boards in online distance learning: A case study - Hernández-García, Ángel; González-González, Inés; Jiménez-Zarco, Ana Isabel; Chaparro-Peláez, Julián) Cited By :53Export Date: 20 September 2020CODEN: CHBEECorrespondence Address: Hernández-García, Á.; Departamento de Ingeniería de Organización, Administración de Empresas y Estadística, Universidad Politécnica de MadridSpainReferences: Ahn, J., What can we learn from Facebook activity? Using social learning analytics to observe new media literacy skills (2013) Proceedings of the Third International Conference on Learning Analytics and Knowledge (LAK ’13), pp. 135-144; Aviv, R., Erlich, Z., Ravid, G., Geva, A., Network analysis of knowledge construction in asynchronous learning networks (2003) Journal of Asynchronous Learning Networks, 7 (3), pp. 1-23; Aviv, R., Erlich, Z., Ravid, G., Cohesion and roles: Network analysis of CSCL communities (2003) Proceedings of the 3rd IEEE International Conference on Advanced Learning Technologies, pp. 145-149. , (ICALT ’03); Bakharia, A., Dawson, S., SNAPP: A bird’s-eye view of temporal participant interaction (2011) Proceedings of the 1st International Conference on Learning Analytics and Knowledge (LAK ’11), pp. 168-173; Beaudoin, M.F., Learning or lurking? Tracking the &quot;invisible&quot; online student (2002) The Internet and Higher Education, 5 (2), pp. 147-155; Buckingham-Shum, S., Ferguson, R., Social learning analytics (2012) Journal of Educational Technology &amp; Society, 15 (3), pp. 3-26; Cambridge, D., Perez-Lopez, K., First steps towards a social learning analytics for online communities of practice for educators (2012) Proceedings of the 2nd International Conference on Learning Analytics and Knowledge (LAK “12), pp. 69-72; Capuano, N., Laria, G., Mazzoni, E., Pierri, A., Mangione G. ., R., Improving role taking in CSCL script using SNA and semantic web (2011) Proceedings of the IEEE 11th International Conference on Advanced Learning Technologies (ICALT ‘11), pp. 636-637; Chang, C.-T., Hsieh, P.-H., The interaction patterns of knowledge sharing in design forums (2012) PACIS 2012 Proceedings, Paper 171; Cho, H., Gay, G., Davidson, B., Ingraffea, A., Social networks, communication styles, and learning performance in a CSCL community (2007) Computers &amp; Education, 49 (2), pp. 309-329; Dawson, S., A study of the relationship between student social networks and sense of community (2008) Educational Technology &amp; Society, 11 (3), pp. 224-238; Freeman, L.C., Centrality in social networks: Conceptual clarification (1978) Social Networks, 1 (3), pp. 215-239; Fruchterman, T.M.J., Reingold, E.M., Graph drawing by force-directed placement (1991) Software: Practice and Experience, 21 (11), pp. 1129-1164; García-Peñalvo, F.J., Colomo-Palacios, R., Lytras, M.D., Informal learning in work environments: Training with the Social Web in the workplace (2012) Behaviour &amp; Information Technology, 31 (8), pp. 753-755; García-Saiz, D., Palazuelos, C., Zorrilla, M., Data mining and social network analysis in the educational field: An application for non-expert users (2013) Educational Data Mining: Applications and Trends, pp. 411-439. , A. Peña-Ayala, Springer, Berlin/Heidelberg Berlin, Heidelberg; Grunspan, D.Z., Wiggins, B.L., Goodreau, S.M., Understanding classrooms through social network analysis: A primer for social network analysis in education research (2014) CBE Life Sciences Education, 13 (2), pp. 167-178; Hernández-García, A., Usare Gephi per Visualizzare la Partecipazione Nei Corsi Online: Un Approccio di Social Learning Analytics, , Tecnologie Didattiche; Huang, E., Lin, S., Huang, T., What type of learning style leads to online participation in the mixed-mode e-learning environment? A study of software usage instruction (2012) Computers &amp; Education, 58, pp. 338-349; Krčadinac, U., Jovanović, J., Devedžić, V., Visualizing the affective structure of students interaction (2012) Hybrid Learning, pp. 23-34. , S.K.S. Cheung, J. Fong, L.-F. Kwok, K. Li, R. Kwan, Berlin/Heidelberg: Springer Berlin Heidelberg; Laat, M., Lally, V., Lipponen, L., Simons, R.J., Investigating patterns of interaction in networked learning and computer-supported collaborative learning: A role for social network analysis (2007) International Journal of Computer-Supported Collaborative Learning, 2 (1), pp. 87-103; Lipponen, L., Rahikainen, M., Lallimo, J., Hakkarainen, K., Patterns of participation and discourse in elementary students’ computer-supported collaborative learning (2003) Learning and Instruction, 13 (5), pp. 487-509; Long, P., Siemens, G., Penetrating the fog: Analytics in learning and education (2011) EDUCAUSE Review, 46 (5), pp. 31-40; Macfadyen, L.P., Dawson, S., Mining LMS data to develop an ‘ “early warning system&quot; for educators: A proof of concept (2010) Computers &amp; Education, 54 (2), pp. 588-599; Macfadyen, L., Dawson, S., Numbers are not enough. Why e-learning analytics failed to inform an institutional strategic plan (2012) Educational Technology &amp; Society, 15 (3), pp. 149-163; Martínez, A., Dimitriadis, Y., Rubia, B., Gómez, E., De La Fuente, P., Combining qualitative evaluation and social network analysis for the study of classroom social interactions (2003) Computers &amp; Education, 41 (4), pp. 353-368; Mazzolini, M., Maddison, S., When to jump in: The role of the instructor in online discussion forums (2007) Computers &amp; Education, 49 (2), pp. 193-213; Nistor, N., Trəuşan-Matu, S., Dascəlu, M., Duttweiler, H., Chiru, C., Baltes, B., Finding student-centered open learning environments on the internet: Automated dialogue assessment in academic virtual communities of practice (2015) Computers in Human Behavior, 47, pp. 119-127; Nurmela, K., Lehtinen, E., Palonen, T., Evaluating CSCL log files by social network analysis (1999) Proceedings of the 1999 Conference on Computer Support for Collaborative Learning (CSCL ‘99), , Article No. 54; (2005) Illuminating the Path. the Research and Development Agenda for Visual Analytics (1st Ed.), , NVAC (National Visualization and Analytics Center). National Visualization and Analytics Center; Pang, S., Reinking, D., Hutchison, A., Ramey, D., (2011) Comparing Teachers’ Perceptions of Integrating Information and Communication Technologies into Literacy Instruction in South Korea and the U.S. Annual Meeting of the Literacy Research Association; Pérez-Sanagustín, M., Alario-Hoyos, C., Kloos, C.D., FLINN: A framework to characterize technology enhanced formal, non-formal and informal learning situations (2014) International Journal of Human Capital and Information Technology Professionals, 5 (2), pp. 38-51; Rabbany, R., Elatia, S., Takaffoli, M., Zaïane, O.R., Collaborative learning of students in online discussion forums: A social network analysis perspective (2013) Educational Data Mining: Applications and Trends, pp. 441-466. , Springer Berlin, Heidelberg; Reffay, C., Chanier, T., How social network analysis can help to measure cohesion in collaborative distance-learning (2003) Designing for Change in Networked Learning Environments: Computer-supported Collaborative Learning (Vol. 2), pp. 343-352. , B. Wasson, S. Ludvigsen, U. Hoppe, Springer Netherlands; Rizzuto, T.E., Ledoux, J., Hatala, J.P., It’s not just what you know, it’s who you know: Testing a model of the relative importance of social networks to academic performance (2008) Social Psychology of Education, 12 (2), pp. 175-189; Romero, C., Lopez, M., Luna, J., Ventura, S., Predicting students” final performance from participation in on-line discussion forums (2013) Computers &amp; Education, 68, pp. 458-472; Siemens, G., Gasevic, D., Haythornthwaite, C., Dawson, S., Buckingham Shum, S., Ferguson, R., Open learning analytics: An integrated &amp; modularized platform (2011) Proposal to Design, Implement and Evaluate An Open Platform to Integrate Heterogeneous Learning Analytics Techniques, , http://solaresearch.org/OpenLearningAnalytics.pdf, Society for Learning Analytics Research (SoLAR). Retrieved from; Sparrowe, R.T., Liden, R.C., Wayne, S.J., Kraimer, M.L., Social networks and the performance of individuals and groups (2001) The Academy of Management Journal, 44 (2), pp. 316-325; Stantchev, V., Colomo-Palacios, R., Soto-Acosta, P., Misra, S., Learning management systems and cloud file hosting services: A study on students’ acceptance (2014) Computers in Human Behavior, 31, pp. 612-619; Tobarra, L., Robles-Gómez, A., Ros, S., Hernández, R., Caminero, A.C., Analyzing the students” behavior and relevant topics in virtual learning communities (2014) Computers in Human Behavior, 31, pp. 659-669; Verbert, K., Duval, E., Klerkx, J., Govaerts, S., Santos, J.L., Learning analytics dashboard applications (2013) American Behavioral Scientist, 57 (10), pp. 1500-1509; Wise A. ., F., Hausknecht S. ., N., Learning analytics for online discussions: A pedagogical model for intervention with embedded and extracted analytics (2013) Proceedings of the Third International Conference on Learning Analytics and Knowledge (LAK ’13), pp. 48-56 From Duplicate 3 (Applying social learning analytics to message boards in online distance learning: A case study - Hernández-García, Ángel; González-González, Inés; Jiménez-Zarco, Ana Isabel; Chaparro-Peláez, Julián) Cited By :53Export Date: 20 September 2020CODEN: CHBEECorrespondence Address: Hernández-García, Á.; Departamento de Ingeniería de Organización, Administración de Empresas y Estadística, Universidad Politécnica de MadridSpainReferences: Ahn, J., What can we learn from Facebook activity? Using social learning analytics to observe new media literacy skills (2013) Proceedings of the Third International Conference on Learning Analytics and Knowledge (LAK ’13), pp. 135-144; Aviv, R., Erlich, Z., Ravid, G., Geva, A., Network analysis of knowledge construction in asynchronous learning networks (2003) Journal of Asynchronous Learning Networks, 7 (3), pp. 1-23; Aviv, R., Erlich, Z., Ravid, G., Cohesion and roles: Network analysis of CSCL communities (2003) Proceedings of the 3rd IEEE International Conference on Advanced Learning Technologies, pp. 145-149. , (ICALT ’03); Bakharia, A., Dawson, S., SNAPP: A bird’s-eye view of temporal participant interaction (2011) Proceedings of the 1st International Conference on Learning Analytics and Knowledge (LAK ’11), pp. 168-173; Beaudoin, M.F., Learning or lurking? Tracking the &quot;invisible&quot; online student (2002) The Internet and Higher Education, 5 (2), pp. 147-155; Buckingham-Shum, S., Ferguson, R., Social learning analytics (2012) Journal of Educational Technology &amp; Society, 15 (3), pp. 3-26; Cambridge, D., Perez-Lopez, K., First steps towards a social learning analytics for online communities of practice for educators (2012) Proceedings of the 2nd International Conference on Learning Analytics and Knowledge (LAK “12), pp. 69-72; Capuano, N., Laria, G., Mazzoni, E., Pierri, A., Mangione G. ., R., Improving role taking in CSCL script using SNA and semantic web (2011) Proceedings of the IEEE 11th International Conference on Advanced Learning Technologies (ICALT ‘11), pp. 636-637; Chang, C.-T., Hsieh, P.-H., The interaction patterns of knowledge sharing in design forums (2012) PACIS 2012 Proceedings, Paper 171; Cho, H., Gay, G., Davidson, B., Ingraffea, A., Social networks, communication styles, and learning performance in a CSCL community (2007) Computers &amp; Education, 49 (2), pp. 309-329; Dawson, S., A study of the relationship between student social networks and sense of community (2008) Educational Technology &amp; Society, 11 (3), pp. 224-238; Freeman, L.C., Centrality in social networks: Conceptual clarification (1978) Social Networks, 1 (3), pp. 215-239; Fruchterman, T.M.J., Reingold, E.M., Graph drawing by force-directed placement (1991) Software: Practice and Experience, 21 (11), pp. 1129-1164; García-Peñalvo, F.J., Colomo-Palacios, R., Lytras, M.D., Informal learning in work environments: Training with the Social Web in the workplace (2012) Behaviour &amp; Information Technology, 31 (8), pp. 753-755; García-Saiz, D., Palazuelos, C., Zorrilla, M., Data mining and social network analysis in the educational field: An application for non-expert users (2013) Educational Data Mining: Applications and Trends, pp. 411-439. , A. Peña-Ayala, Springer, Berlin/Heidelberg Berlin, Heidelberg; Grunspan, D.Z., Wiggins, B.L., Goodreau, S.M., Understanding classrooms through social network analysis: A primer for social network analysis in education research (2014) CBE Life Sciences Education, 13 (2), pp. 167-178; Hernández-García, A., Usare Gephi per Visualizzare la Partecipazione Nei Corsi Online: Un Approccio di Social Learning Analytics, , Tecnologie Didattiche; Huang, E., Lin, S., Huang, T., What type of learning style leads to online participation in the mixed-mode e-learning environment? A study of software usage instruction (2012) Computers &amp; Education, 58, pp. 338-349; Krčadinac, U., Jovanović, J., Devedžić, V., Visualizing the affective structure of students interaction (2012) Hybrid Learning, pp. 23-34. , S.K.S. Cheung, J. Fong, L.-F. Kwok, K. Li, R. Kwan, Berlin/Heidelberg: Springer Berlin Heidelberg; Laat, M., Lally, V., Lipponen, L., Simons, R.J., Investigating patterns of interaction in networked learning and computer-supported collaborative learning: A role for social network analysis (2007) International Journal of Computer-Supported Collaborative Learning, 2 (1), pp. 87-103; Lipponen, L., Rahikainen, M., Lallimo, J., Hakkarainen, K., Patterns of participation and discourse in elementary students’ computer-supported collaborative learning (2003) Learning and Instruction, 13 (5), pp. 487-509; Long, P., Siemens, G., Penetrating the fog: Analytics in learning and education (2011) EDUCAUSE Review, 46 (5), pp. 31-40; Macfadyen, L.P., Dawson, S., Mining LMS data to develop an ‘ “early warning system&quot; for educators: A proof of concept (2010) Computers &amp; Education, 54 (2), pp. 588-599; Macfadyen, L., Dawson, S., Numbers are not enough. Why e-learning analytics failed to inform an institutional strategic plan (2012) Educational Technology &amp; Society, 15 (3), pp. 149-163; Martínez, A., Dimitriadis, Y., Rubia, B., Gómez, E., De La Fuente, P., Combining qualitative evaluation and social network analysis for the study of classroom social interactions (2003) Computers &amp; Education, 41 (4), pp. 353-368; Mazzolini, M., Maddison, S., When to jump in: The role of the instructor in online discussion forums (2007) Computers &amp; Education, 49 (2), pp. 193-213; Nistor, N., Trəuşan-Matu, S., Dascəlu, M., Duttweiler, H., Chiru, C., Baltes, B., Finding student-centered open learning environments on the internet: Automated dialogue assessment in academic virtual communities of practice (2015) Computers in Human Behavior, 47, pp. 119-127; Nurmela, K., Lehtinen, E., Palonen, T., Evaluating CSCL log files by social network analysis (1999) Proceedings of the 1999 Conference on Computer Support for Collaborative Learning (CSCL‘99), , Article No. 54; (2005) Illuminating the Path. the Research and Development Agenda for Visual Analytics (1st Ed.), , NVAC (National Visualization and Analytics Center). National Visualization and Analytics Center; Pang, S., Reinking, D., Hutchison, A., Ramey, D., (2011) Comparing Teachers’ Perceptions of Integrating Information and Communication Technologies into Literacy Instruction in South Korea and the U.S. Annual Meeting of the Literacy Research Association; Pérez-Sanagustín, M., Alario-Hoyos, C., Kloos, C.D., FLINN: A framework to characterize technology enhanced formal, non-formal and informal learning situations (2014) International Journal of Human Capital and Information Technology Professionals, 5 (2), pp. 38-51; Rabbany, R., Elatia, S., Takaffoli, M., Zaïane, O.R., Collaborative learning of students in online discussion forums: A social network analysis perspective (2013) Educational Data Mining: Applications and Trends, pp. 441-466. , Springer Berlin, Heidelberg; Reffay, C., Chanier, T., How social network analysis can help to measure cohesion in collaborative distance-learning (2003) Designing for Change in Networked Learning Environments: Computer-supported Collaborative Learning (Vol. 2), pp. 343-352. , B. Wasson, S. Ludvigsen, U. Hoppe, Springer Netherlands; Rizzuto, T.E., Ledoux, J., Hatala, J.P., It’s not just what you know, it’s who you know: Testing a model of the relative importance of social networks to academic performance (2008) Social Psychology of Education, 12 (2), pp. 175-189; Romero, C., Lopez, M., Luna, J., Ventura, S., Predicting students” final performance from participation in on-line discussion forums (2013) Computers &amp; Education, 68, pp. 458-472; Siemens, G., Gasevic, D., Haythornthwaite, C., Dawson, S., Buckingham Shum, S., Ferguson, R., Open learning analytics: An integrated &amp; modularized platform (2011) Proposal to Design, Implement and Evaluate An Open Platform to Integrate Heterogeneous Learning Analytics Techniques, , http://solaresearch.org/OpenLearningAnalytics.pdf, Society for Learning Analytics Research (SoLAR). Retrieved from; Sparrowe, R.T., Liden, R.C., Wayne, S.J., Kraimer, M.L., Social networks and the performance of individuals and groups (2001) The Academy of Management Journal, 44 (2), pp. 316-325; Stantchev, V., Colomo-Palacios, R., Soto-Acosta, P., Misra, S., Learning management systems and cloud file hosting services: A study on students’ acceptance (2014) Computers in Human Behavior, 31, pp. 612-619; Tobarra, L., Robles-Gómez, A., Ros, S., Hernández, R., Caminero, A.C., Analyzing the students” behavior and relevant topics in virtual learning communities (2014) Computers in Human Behavior, 31, pp. 659-669; Verbert, K., Duval, E., Klerkx, J., Govaerts, S., Santos, J.L., Learning analytics dashboard applications (2013) American Behavioral Scientist, 57 (10), pp. 1500-1509; Wise A. ., F., Hausknecht S. ., N., Learning analytics for online discussions: A pedagogical model for intervention with embedded and extracted analytics (2013) Proceedings of the Third International Conference on Learning Analytics and Knowledge (LAK ’13), pp. 48-56 From Duplicate 4 (Applying social learning analytics to message boards in online distance learning: A case study - Hernández-García, Ángel; González-González, Inés; Jiménez-Zarco, Ana Isabel; Chaparro-Peláez, Julián) From Duplicate 1 (Applying social learning analytics to message boards in online distance learning: A case study - Hernández-García, Ángel; González-González, Inés; Jiménez-Zarco, Ana Isabel; Chaparro-Peláez, Julián) Cited By :53Export Date: 20 September 2020CODEN: CHBEECorrespondence Address: Hernández-García, Á.; Departamento de Ingeniería de Organización, Administración de Empresas y Estadística, Universidad Politécnica de MadridSpainReferences: Ahn, J., What can we learn from Facebook activity? Using social learning analytics to observe new media literacy skills (2013) Proceedings of the Third International Conference on Learning Analytics and Knowledge (LAK ’13), pp. 135-144; Aviv, R., Erlich, Z., Ravid, G., Geva, A., Network analysis of knowledge construction in asynchronous learning networks (2003) Journal of Asynchronous Learning Networks, 7 (3), pp. 1-23; Aviv, R., Erlich, Z., Ravid, G., Cohesion and roles: Network analysis of CSCL communities (2003) Proceedings of the 3rd IEEE International Conference on Advanced Learning Technologies, pp. 145-149. , (ICALT ’03); Bakharia, A., Dawson, S., SNAPP: A bird’s-eye view of temporal participant interaction (2011) Proceedings of the 1st International Conference on Learning Analytics and Knowledge (LAK ’11), pp. 168-173; Beaudoin, M.F., Learning or lurking? Tracking the &quot;invisible&quot; online student (2002) The Internet and Higher Education, 5 (2), pp. 147-155; Buckingham-Shum, S., Ferguson, R., Social learning analytics (2012) Journal of Educational Technology &amp; Society, 15 (3), pp. 3-26; Cambridge, D., Perez-Lopez, K., First steps towards a social learning analytics for online communities of practice for educators (2012) Proceedings of the 2nd International Conference on Learning Analytics and Knowledge (LAK ’12), pp. 69-72; Capuano, N., Laria, G., Mazzoni, E., Pierri, A., Mangione G. ., R., Improving role taking in CSCL script using SNA and semantic web (2011) Proceedings of the IEEE 11th International Conference on Advanced Learning Technologies (ICALT ’11), pp. 636-637; Chang, C.-T., Hsieh, P.-H., The interaction patterns of knowledge sharing in design forums (2012) PACIS 2012 Proceedings, Paper 171; Cho, H., Gay, G., Davidson, B., Ingraffea, A., Social networks, communication styles, and learning performance in a CSCL community (2007) Computers &amp; Education, 49 (2), pp. 309-329; Dawson, S., A study of the relationship between student social networks and sense of community (2008) Educational Technology &amp; Society, 11 (3), pp. 224-238; Freeman, L.C., Centrality in social networks: Conceptual clarification (1978) Social Networks, 1 (3), pp. 215-239;} }

@article{Holme_2015, title={Modern temporal network theory: a colloquium}, volume={88}, ISSN={1434-6036}, url={http://dx.doi.org/10.1140/epjb/e2015-60657-4}, DOI={10.1140/epjb/e2015-60657-4}, abstractNote={The power of any kind of network approach lies in the ability to simplify a complex system so that one can better understand its function as a whole. Sometimes it is beneficial, however, to include more information than in a simple graph of only nodes and links. Adding information about times of interactions can make predictions and mechanistic understanding more accurate. The drawback, however, is that there are not so many methods available, partly because temporal networks is a relatively young field, partly because it is more difficult to develop such methods compared to for static networks. In this colloquium, we review the methods to analyze and model temporal networks and processes taking place on them, focusing mainly on the last three years. This includes the spreading of infectious disease, opinions, rumors, in social networks; information packets in computer networks; various types of signaling in biology, and more. We also discuss future directions.}, number={9}, journal={European Physical Journal B: Condensed Matter and Complex Systems}, author={Holme, Petter}, year={2015} }

@article{Holme_Saramaki_2012, title={Temporal networks}, volume={519}, ISSN={0370-1573}, abstractNote={A great variety of systems in nature, society and technology-from the web of sexual contacts to the Internet, from the nervous system to power grids-can be modeled as graphs of vertices coupled by edges. The network structure, describing how the graph is wired, helps us understand, predict and optimize the behavior of dynamical systems. In many cases, however, the edges are not continuously active. As an example, in networks of communication via e-mail, text messages, or phone calls, edges represent sequences of instantaneous or practically instantaneous contacts. In some cases, edges are active for non-negligible periods of time: e.g.,the proximity patterns of inpatients at hospitals can be represented by a graph where an edge between two individuals is on throughout the time they are at the same ward. Like network topology, the temporal structure of edge activations can affect dynamics of systems interacting through the network, from disease contagion on the network of patients to information diffusion over an e-mail network. In this review, we present the emergent field of temporal networks, and discuss methods for analyzing topological and temporal structure and models for elucidating their relation to the behavior of dynamical systems. In the light of traditional network theory, one can see this framework as moving the information of when things happen from the dynamical system on the network, to the network itself. Since fundamental properties, such as the transitivity of edges, do not necessarily hold in temporal networks, many of these methods need to be quite different from those for static networks. The study of temporal networks is very interdisciplinary in nature. Reflecting this, even the object of study has many names-temporal graphs, evolving graphs, time-varying graphs, time-aggregated graphs, time-stamped graphs, dynamic networks, dynamic graphs, dynamical graphs, and so on. This review covers different fields where temporal graphs are considered, but does not attempt to unify related terminology-rather, we want to make papers readable across disciplines. © 2012 Elsevier B.V.}, number={3}, journal={Physics reports}, publisher={Elsevier B.V.}, author={Holme, Petter and Saramäki, Jari}, year={2012}, pages={97–125} }

@inbook{Holme_Saramäki_2019, title={A Map of Approaches to Temporal Networks}, author={Holme, Petter and Saramäki, Jari}, year={2019}, pages={1–24} }

@article{Johnson_Azevedo_DMello_2011, title={The Temporal and Dynamic Nature of Self-Regulatory Processes During Independent and Externally Assisted Hypermedia Learning}, volume={29}, ISSN={0737-0008}, number={4}, journal={Cognition and instruction}, publisher={Routledge}, author={Johnson, Amy M. and Azevedo, Roger and D’Mello, Sidney K.}, year={2011}, month={Oct}, pages={471–504}, annote={doi: 10.1080/07370008.2011.610244} }

@article{Li_Cornelius_Liu_Wang_Barabási_2017, title={The fundamental advantages of temporal networks}, volume={358}, ISSN={0036-8075}, abstractNote={Most networked systems of scientific interest are characterized by temporal links, meaning the network’s structure changes over time. Link temporality has been shown to hinder many dynamical processes, from information spreading to accessibility, by disrupting network paths. Considering the ubiquity of temporal networks in nature, we ask: Are there any advantages of the networks’ temporality? We use an analytical framework to show that temporal networks can, compared to their static counterparts, reach controllability faster, demand orders of magnitude less control energy, and have control trajectories, that are considerably more compact than those characterizing static networks. Thus, temporality ensures a degree of flexibility that would be unattainable in static networks, enhancing our ability to control them.}, number={6366}, journal={Science}, author={Li, A. and Cornelius, S. P. and Liu, Y-Y and Wang, L. and Barabási, A-L}, year={2017}, month={Nov}, pages={1042–1046}, language={en} }

@article{Lopez-Pernas_Saqr_2021, title={Bringing synchrony and clarity to complex multi-channel data: A learning analytics study in programming education}, ISSN={2169-3536}, abstractNote={Supporting teaching and learning programming with learning analytics is an active area of inquiry. Most learning management systems were not developed to support learning programming. Therefore, educators have to resort to other systems that support the programming process, which can pose a challenge when it comes to understanding students’ learning since it takes place in different contexts. Methods that support the combination of different data sources are needed. Such methods would ideally account for the time-ordered sequence of students’ learning actions. In this article, we use a novel method (multi-channel sequence mining with Hidden Markov Models, HMMs) that allows the combination of multiple data sources, accounts for the temporal nature of students’ learning actions, and maps the transitions between different learning tactics. Our study included 291 students enrolled in a higher education programming course. Students’ trace-log data were collected from the learning management system and from a programming automated assessment tool. Data were analyzed using multi-channel sequence mining and HMM. The results reveal different patterns of students’ approaches to learning programming. High achievers start earlier to work on the programming assignments, use more independent strategies and consume learning resources more frequently, while the low achievers procrastinate early in the course and rely on help forums. Our findings demonstrate the potentials of multi-channel sequence mining and how this method can be analyzed using HMM. Furthermore, the results obtained can be of use for educators to understand students’ strategies when learning programming.}, journal={IEEE Access}, author={Lopez-Pernas, Sonsoles and Saqr, Mohammed}, year={2021}, pages={1–1}, keywords={Learning Analytics;Programming;Computer Science Education;Sequence Mining;Hidden Markov Models;Automated Assessment} }

@inbook{Lopez-Pernas_Saqr_Del, title={A broad collection of datasets for educational research training and application}, booktitle={Learning analytics methods and tutorials: A practical guide using R}, publisher={Springer}, author={Lopez-Pernas, Sonsoles and Saqr, Mohammed and Del Rio, Laura}, editor={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2024}, pages={in–press} }

@article{Lopez-Pernas_Saqr_Gordillo_Barra_2022, title={A learning analytics perspective on educational escape rooms}, ISSN={1049-4820}, abstractNote={ABSTRACTLearning analytics methods have proven useful in providing insights from the increasingly available digital data about students in a variety of learning environments, including serious games. However, such methods have not been applied to the specific context of educational escape rooms and therefore little is known about students’ behavior while playing. The present work aims to fill the gap in the existing literature by showcasing the power of learning analytics methods to reveal and represent students’ behavior when participating in a computer-supported educational escape room. Specifically, we make use of sequence mining methods to analyze the temporal and sequential aspects of the activities carried out by students during these novel educational games. We further use clustering to identify different player profiles according to the sequential unfolding of students’ actions and analyze how these profiles relate to knowledge acquisition. Our results show that students’ behavior differed significantly in their use of hints in the escape room and resulted in differences in their knowledge acquisition levels.}, journal={Interactive Learning Environments}, publisher={Routledge}, author={Lopez-Pernas, Sonsoles and Saqr, Mohammed and Gordillo, Aldo and Barra, Enrique}, year={2022}, month={Feb}, pages={1–17} }

@inbook{Nicosia_Tang_Mascolo_Musolesi_Russo_Latora_2013, title={Graph metrics for temporal networks}, booktitle={Temporal networks}, publisher={Springer}, author={Nicosia, Vincenzo and Tang, John and Mascolo, Cecilia and Musolesi, Mirco and Russo, Giovanni and Latora, Vito}, year={2013}, pages={15–40} }

@inproceedings{Peeters_Saqr_Viberg_2020, title={Applying Learning Analytics to Map Students ’ Self-Regulated Learning Tactics in an Academic Writing Course}, author={Peeters, Ward and Saqr, Mohammed and Viberg, Olga}, year={2020} }

@inproceedings{Poquet_Saqr_Chen_2021, title={Recommendations for Network Research in Learning Analytics: To Open a Conversation}, booktitle={Proceedings of the NetSciLA21 workshop}, author={Poquet, Oleksandra and Saqr, Mohammed and Chen, Bodong}, year={2021} }

@article{Reimann_2009, title={Time is precious: Variable- and event-centred approaches to process analysis in CSCL research}, volume={4}, ISSN={1556-1615}, abstractNote={Although temporality is a key characteristic of the core concepts of CSCL-interaction, communication, learning, knowledge building, technology use-and although CSCL researchers have privileged access to process data, the theoretical constructs and methods employed in research practice frequently neglect to make full use of information relating to time and order. This is particularly problematic when collaboration and learning processes are studied in groups that work together over weeks, and months, as is often the case. The quantitative method dominant in the social and learning sciences-variable-centred variance theory-is of limited value for studying change on longer time scales. We introduce the event-centred view of process as a more generally applicable approach, not only for quantitative analysis, but also for providing closer links between qualitative and quantitative research methods. A number of methods for variable- and event-centred analysis of process data are described and compared, using examples from CSCL research. I conclude with suggestions on how experimental, descriptive, and design-oriented research orientations can become better integrated. © International Society of the Learning Sciences, Inc.; Springer Science + Business Media, LLC 2009.}, number={3}, journal={International Journal of Computer-Supported Collaborative Learning}, author={Reimann, Peter}, year={2009}, pages={239–257}, keywords={Process analysis; Qualitative methods; Quantitative methods; Research methods} }

@article{Saqr_Elmoazen_Tedre_Lopez-Pernas_Hirsto_2022, title={How well centrality measures capture student achievement in computer-supported collaborative learning? – A systematic review and meta-analysis}, volume={35}, ISSN={1747-938X}, abstractNote={Research has shown the value of social collaboration and the benefits it brings to learners. In this study, we investigate the worth of Social Network Analysis (SNA) in translating students’ interactions in computer-supported collaborative learning (CSCL) into proxy indicators of achievement. Previous research has tested the correlation between SNA centrality measures and achievement. Some results indicate a positive association, while others do not. To synthesize research efforts, investigate which measures are of value, and how strong of an association exists, this article presents a systematic review and meta-analysis of 19 studies that included 33 cohorts and 16 centrality measures. Achievement was operationalized in most of the reviewed studies as final course or task grade. All studies reported that one or more centrality measures had a positive and significant correlation with, or a potential for predicting, achievement. Every centrality measure in the reviewed sample has shown a positive correlation with achievement in at least one study. In all the reviewed studies, degree centralities correlated with achievement in terms of final course grades or other achievement measure with the highest magnitude. Eigenvector-based centralities (Eigenvector, PageRank, hub, and authority values) were also positively correlated and mostly statistically significant in all the reviewed studies. These findings emphasize the robustness and reliability of degree- and eigenvector-based centrality measures in understanding students’ interactions in relation to achievement. In contrast, betweenness and closeness centralities have shown mixed or weak correlations with achievement. Taken together, our findings support the use of centrality measures as valid proxy indicators of academic achievement and their utility for monitoring interactions in collaborative learning settings.}, journal={Educational Research Review}, author={Saqr, Mohammed and Elmoazen, Ramy and Tedre, Matti and Lopez-Pernas, Sonsoles and Hirsto, Laura}, year={2022}, month={Feb}, pages={100437}, keywords={Centrality measures; CSCL; Achievement; Social network analysis; Learning analytics; Predicting performance; Educational data mining} }

@inproceedings{Saqr_Lopez-Pernas_2022a, title={Instant or Distant: A Temporal Network Tale of Two Interaction Platforms and Their Influence on Collaboration}, abstractNote={This study compared two iterations of the same course where students had the same assignments. In the first iteration, the students had to use the typical discussion forums offered by the popular Moodle learning management system. In the second iteration, students had to use Discord, the popular gaming chat application. Students’ interactions were retrieved from both platforms and cleaned. Two social networks were constructed using the same methods to evaluate the differences in patterns of interaction between the two platforms, the group interactivity, the reciprocity, and the quality of interactions. The aim is to study how far an instant messenger facilitates or otherwise constrains collaboration. We use temporal network methods to further understand the pace, rhythm, and temporality of interactions.}, booktitle={Educating for a New Future: Making Sense of Technology-Enhanced Learning Adoption}, publisher={Springer International Publishing}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2022}, pages={594–600} }

@inproceedings{Saqr_Lopez-Pernas_2022b, title={The why, the what and the how to model a dynamic relational learning process with temporal networks}, url={https://www.researchgate.net/profile/Mohammed-Saqr/publication/364997941_The_Why_the_What_and_the_How_to_Model_a_Dynamic_Relational_Learning_Process_with_Temporal_Networks/links/636271222f4bca7fd0270b74/The-Why-the-What-and-the-How-to-Model-a-Dynamic-Relational-Learning-Process-with-Temporal-Networks.pdf}, booktitle={Proceedings of the NetSciLA22 workshop}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2022} }

@article{Saqr_Lopez-Pernas_2022c, title={The curious case of centrality measures: A large-scale empirical investigation}, volume={9}, ISSN={1929-7750}, abstractNote={There has been extensive research using centrality measures in educational settings. One of the most common lines of such research has tested network centrality measures as indicators of success. The increasing interest in centrality measures has been kindled by the proliferation of learning analytics. Previous works have been dominated by single-course case studies that have yielded inconclusive results regarding the consistency and suitability of centrality measures as indicators of academic achievement. Therefore, large-scale studies are needed to overcome the multiple limitations of existing research (limited datasets, selective and reporting bias, as well as limited statistical power). This study aims to empirically test and verify the role of centrality measures as indicators of success in collaborative learning. For this purpose, we attempted to reproduce the most commonly used centrality measures in the literature in all the courses of an institution over five years of education. The study included a large dataset (n=3,277) consisting of 69 course offerings, with similar pedagogical underpinnings, using meta-analysis as a method to pool the results of different courses. Our results show that degree and eigenvector centrality measures can be a consistent indicator of performance in collaborative settings. Betweenness and closeness centralities yielded uncertain predictive intervals and were less likely to replicate. Our results have shown moderate levels of heterogeneity, indicating some diversity of the results comparable to single laboratory replication studies.}, number={1}, journal={Journal of learning analytics}, publisher={Society for Learning Analytics Research}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2022}, month={Mar}, pages={13–31} }

@article{Saqr_Lopez-Pernas_2022d, title={How CSCL roles emerge, persist, transition, and evolve over time: A four-year longitudinal study}, volume={189}, ISSN={0360-1315}, number={104581}, journal={Computers & education}, publisher={Elsevier BV}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2022}, month={Nov}, pages={104581}, language={en} }

@article{Saqr_Lopez-Pernas_2023, title={The temporal dynamics of online problem-based learning: Why and when sequence matters}, volume={18}, ISSN={1556-1615}, abstractNote={Early research on online PBL explored student satisfaction, effectiveness, and design. The temporal aspect of online PBL has rarely been addressed. Thus, a gap exists in our knowledge regarding how online PBL unfolds: when and for how long a group engages in collaborative discussions. Similarly, little is known about whether and what sequence of interactions could predict higher achievement. This study aims to bridge such a gap by implementing the latest advances in temporal learning analytics to analyze the sequential and temporal aspects of online PBL across a large sample (n = 204 students) of qualitatively coded interactions (8,009 interactions). We analyzed interactions at the group level to understand the group dynamics across whole problem discussions, and at the student level to understand the students’ contribution dynamics across different episodes. We followed such analyses by examining the association of interaction types and the sequences thereof with students’ performance using multilevel linear regression models. The analysis of the interactions reflected that the scripted PBL process is followed a logical sequence, yet often lacked enough depth. When cognitive interactions (e.g., arguments, questions, and evaluations) occurred, they kindled high cognitive interactions, when low cognitive and social interactions dominated, they kindled low cognitive interactions. The order and sequence of interactions were more predictive of performance, and with a higher explanatory power as compared to frequencies. Starting or initiating interactions (even with low cognitive content) showed the highest association with performance, pointing to the importance of initiative and sequencing.}, number={1}, journal={International Journal of Computer-Supported Collaborative Learning}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2023}, month={Mar}, pages={11–37} }

@article{Saqr_Lopez-Pernas_Jovanović_Gašević_2023, title={Intense, turbulent, or wallowing in the mire: A longitudinal study of cross-course online tactics, strategies, and trajectories}, volume={57}, ISSN={1096-7516}, abstractNote={Research has repeatedly demonstrated that students with effective learning strategies are more likely to have better academic achievement. Existing research has mostly focused on a single course or two, while longitudinal studies remain scarce. The present study examines the longitudinal sequence of students’ strategies, their succession, consistency, temporal unfolding, and whether students tend to retain or adapt strategies between courses. We use a large dataset of online traces from 135 students who completed 10 successive courses (i.e., 1350 course enrollments) in a higher education program. The methods used in this study have shown the feasibility of using trace data recorded by learning management systems to unobtrusively trace and model the longitudinal learning strategies across a program. We identified three program-level strategy trajectories: a stable and intense trajectory related to deep learning where students used diverse strategies and scored the highest grades; a fluctuating interactive trajectory, where students focused on course requirements, scored average grades, and were relatively fluctuating; and a light trajectory related to surface learning where students invested the least effort, scored the lowest grades, and had a relatively stable pathway. Students who were intensely active were more likely to transfer the intense strategies and therefore, they were expected to require less support or guidance. Students focusing on course requirements were not as effective self-regulators as they seemed and possibly required early guidance and support from teachers. Students with consistent light strategies or low effort needed proactive guidance and support.}, journal={The Internet and Higher Education}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles and Jovanović, Jelena and Gašević, Dragan}, year={2023}, month={Apr}, pages={100902}, keywords={Learning analytics; Learning strategies; Sequence analysis; Longitudinal studies} }

@inbook{Saqr_Angel2024, title={Social Network Analysis: A primer, a guide and a tutorial in R}, booktitle={Learning analytics methods and tutorials: A practical guide using R}, publisher={Springer}, author={Saqr, Mohammed and Lopez-Pernas, Sonsoles and Miguel Ángel Conde and Hernández-García, Ángel}, editor={Saqr, Mohammed and Lopez-Pernas, Sonsoles}, year={2024}, pages={in–press} }

@inproceedings{Saqr_Nouri_2020, address={New York, NY, USA}, title={High resolution temporal network analysis to understand and improve collaborative learning}, ISBN={9781450377126}, abstractNote={There has been significant efforts in studying collaborative and social learning using aggregate networks. Such efforts have demonstrated the worth of the approach by providing insights about the interactions, student and teacher roles, and predictability of performance. However, using an aggregated network discounts the fine resolution of temporal interactions. By doing so, we might overlook the regularities/irregularities of students’ interactions, the process of learning regulation, and how and when different actors influence each other. Thus, compressing a complex temporal process such as learning may be oversimplifying and reductionist. Through a temporal network analysis of 54 students interactions (in total 3134 interactions) in an online medical education course, this study contributes with a methodological approach to building, visualizing and quantitatively analyzing temporal networks, that could help educational practitioners understand important temporal aspects of collaborative learning that might need attention and action. Furthermore, the analysis conducted emphasize the importance of considering the time characteristics of the data that should be used when attempting to, for instance, implement early predictions of performance and early detection of students and groups that need support and attention.}, booktitle={Proceedings of the Tenth International Conference on Learning Analytics & Knowledge}, publisher={ACM}, author={Saqr, Mohammed and Nouri, Jalal}, year={2020}, month={Mar}, pages={314–319}, keywords={Collaborative learning; Learning analytics; Medical education; Problem-based learning; Social network analysis; Temporal networks; Temporarily; collaborative learning; learning analytics; problem-based learning; social network analysis; temporal networks; temporarily} }

@article{Saqr_Peeters_2022, title={Temporal networks in collaborative learning: A case study}, ISSN={0007-1013}, url={https://onlinelibrary.wiley.com/doi/10.1111/bjet.13187}, DOI={10.1111/bjet.13187}, abstractNote={Abstract Social Network Analysis (SNA) has enabled researchers to understand and optimize the key dimensions of collaborative learning. A majority of SNA research has so far used static networks, ie, aggregated networks that compile interactions without considering when certain activities or relationships occurred. Compressing a temporal process by discarding time, however, may result in reductionist oversimplifications. In this study, we demonstrate the potentials of temporal networks in the analysis of online peer collaboration. In particular, we study: (1) social interactions by analysing learners’ collaborative behaviour, part of a case study in which they worked on academic writing tasks, and (2) cognitive interactions through the analysis of students’ self-regulated learning tactics. The study included 123 students and 2550 interactions. By using temporal networks, we show how to analyse the longitudinal evolution of a collaborative network visually and quantitatively. Correlation coefficients with grades, when calculated with time-respecting temporal measures of centrality, were more correlated with learning outcomes than traditional centrality measures. Using temporal networks to analyse the co-temporal and longitudinal development, reach, and diffusion patterns of students’ learning tactics has provided novel insights into the complex dynamics of learning, not commonly offered through static networks.}, journal={British Journal of Educational Technology}, publisher={Wiley}, author={Saqr, Mohammed and Peeters, Ward}, year={2022}, month={Feb}, language={en} }

@article{Saqr_Peeters_Viberg_2021, title={The relational, co-temporal, contemporaneous, and longitudinal dynamics of self-regulation for academic writing}, volume={16}, ISSN={1793-7078}, abstractNote={Writing in an academic context often requires students in higher education to acquire a new set of skills while familiarising themselves with the goals, objectives and requirements of the new learning environment. Students’ ability to continuously self-regulate their writing process, therefore, is seen as a determining factor in their learning success. In order to study students’ self-regulated learning (SRL) behaviour, research has increasingly been tapping into learning analytics (LA) methods in recent years, making use of multimodal trace data that can be obtained from students writing and working online. Nevertheless, little is still known about the ways students apply and govern SRL processes for academic writing online, and about how their SRL behaviour might change over time. To provide new perspectives on the use of LA approaches to examine SRL, this study applied a range of methods to investigate what they could tell us about the evolution of SRL tactics and strategies on a relational, co-temporal, contemporaneous and longitudinal level. The data originates from a case study in which a private Facebook group served as an online collaboration space in a first-year academic writing course for foreign language majors of English. The findings show that learners use a range of SRL tactics to manage their writing tasks and that different tactic can take up key positions in this process over time. Several shifts could be observed in students’ behaviour, from mainly addressing content-specific topics to more form-specific and social ones. Our results have also demonstrated that different methods can be used to study the relational, co-temporal, contemporaneous, and longitudinal dynamics of self-regulation in this regard, demonstrating the wealth of insights LA methods can bring to the table.}, number={1}, journal={Research and Practice in Technology Enhanced Learning}, author={Saqr, Mohammed and Peeters, Ward and Viberg, Olga}, year={2021}, month={Oct}, pages={29} }

@article{Vartiainen_Lopez-Pernas_Saqr_Kahila_Parkki_Tedre_Valtonen_2022, title={Mapping students’ temporal pathways in a computational thinking escape room}, volume={1613}, journal={Proceedings http://ceur-ws. org ISSN}, author={Vartiainen, Henriikka and Lopez-Pernas, Sonsoles and Saqr, Mohammed and Kahila, Juho and Parkki, Tuomo and Tedre, Matti and Valtonen, Teemu}, year={2022}, pages={0073} }

@article{Vu_Pattison_Robins_2015, title={Relational event models for social learning in MOOCs}, volume={43}, ISSN={0378-8733}, abstractNote={We propose three extensions for the relational event framework to model the co-evolution of multiple network event streams which are increasingly available thanks to the explosive growth of online applications. Firstly, a flexible stratification approach is considered to allow for more complex data structures with many types of nodes and events. Secondly, an inference method that combines nested case-control sampling with stratification is discussed to scale the approach to very large data sets. Finally, a suite of new temporal and network statistics is introduced to reflect the potentially complex dependencies among events and observed heterogeneities on nodes and edges.The empirical value of new extensions is demonstrated through an analysis of social learning in Massive Open Online Courses (MOOCs). In particular, three modeling problems are considered from the network perspective: (1) the utility of social factors, performance indicators, and clickstream behaviors in the prediction of course dropout, (2) the social and temporal structure of learner interactions across discussion threads, and (3) the forms of mutual dependence of social learning interactions on prior learning success, and future learning success on forms of prior social learning interaction.}, journal={Social networks}, publisher={Elsevier B.V.}, author={Vu, Duy and Pattison, Philippa and Robins, Garry}, year={2015}, pages={121–135}, keywords={MOOCs; Relational event models; Social learning analytics} }


==> title.tex <==
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$

$if(subtitle)$
\subtitle{$subtitle$}
$endif$

$for(by-author)$
  \author{$by-author.name.literal$}
  $if(by-author.affiliations)$
    $for(by-author.affiliations)$
      \affil{%
        $if(by-author.affiliations.name)$
          $by-author.affiliations.name$
        $endif$
      }
    $endfor$
  $endif$
$endfor$
